Linear Arrangement of Halin Graphs

We study the Optimal Linear Arrangement (OLA) problem of Halin graphs, one of the simplest classes of non-outerplanar graphs. We present several properties of OLA of general Halin graphs. We prove a lower bound on the cost of OLA of any Halin graph, and define classes of Halin graphs for which the cost of OLA matches this lower bound. We show for these classes of Halin graphs, OLA can be computed in O(n log n), where n is the number of vertices.

==> branch-one-side.tex <==
Using the fact~\ref{subbranch-two-connected} and also the fact that each spinal branch has exactly two edges from $C$ connected to the rest of the graph, it's not hard to see that for an OLA $\vfi^{*}$ vertices of a branch $B_{i,j}$ cannot be spread around $w_i$.

\noindent
We only consider the case where $\vfi^{*}(w_i) > \vfi^{*}(v_{i,j})$. In contrast with $\vfi^{*}$, we present the modified layout $\vfi^{\diamond}$ defined as:
\[
 \forall v \in V, \vfi^{\diamond} =
    \begin{cases}
       \vfi^{*}(v) + 1 &\quad \text{if }  \vfi^{*}(\underline{v}) \le \vfi^{*}(v) <  \vfi^{*}(w_i)\\
       \vfi^{*}(\underline{v}) &\quad \text{if }  v = w_i\\
       \vfi^{*}(v) &\quad \text{otherwise} \
     \end{cases}
\]
Where $\underline{v} \in V(B_{i,j})$ is the vertex in $B_{i,j}$ labeled with the smallest integer based on $\vfi^{*}$.
Simply in $\vfi^{\diamond}$ all the vertices labeled between $\vfi^{*}(\underline{v})-1$ and $\vfi^{*}(w_i)$ are shifted to the right side of $w_i$.
\footnote{Notice that there may be vertices not in $V(B_{i,j})$ labeled between $\vfi^{*}(\underline{v})-1$ and $w_i$ and their label will be shifted in $vfi^{\diamond}$}.
Aggregating the changes in the expand of all the edges based on the construction of $\vfi^{\diamond}$, it is not hard to see that
$LA(\vfi^{\diamond}) < LA(\vfi^{*})$.
The details and arithmetic calculations are left to the reader.

